MuCol Milestone Report No. 5: Preliminary Parameters

This document is comprised of a collection of updated preliminary parameters for the key parts of the muon collider. The updated preliminary parameters follow on from the October 2023 Tentative Parameters Report. Particular attention has been given to regions of the facility that are believed to hold greater technical uncertainty in their design and that have a strong impact on the cost and power consumption of the facility. The data is collected from a collaborative spreadsheet and transferred to overleaf.

==> Chapters/M-Physics/physics.tex <==
\section{Physics}
\label{phys:sec}


\begin{table}[h]
\begin{center}
\caption{Preliminary summary of the ``baseline'' and ``aspirational'' targets for selected key metrics, reported separately for machines taking data at $\sqrt{s}=3$~TeV and $\sqrt{s}=10$~TeV. The reported performance targets refer to the measurement of the reconstructed objects in physics events after, for example, background subtraction and not to the bare detector performance.}
\label{tab:detector_req}
\begin{tabular}{lccc}
\hline\hline
 \textbf{Requirement} & \multicolumn{2}{c}{\textbf{Baseline}} & \textbf{Aspirational}\\
  & \textbf{$\sqrt{s}=3$~TeV} & \textbf{$\sqrt{s}=10$~TeV} & \\
\hline
Angular acceptance & & & \\
Minimum tracking distance [cm] & & & \\
Forward muons ($\eta> 5$) & & & \\
Track $\sigma_{p_T}/p^{2}_{T}$ [GeV$^{-1}$] & & & \\
Photon energy resolution & & & \\
Neutral hadron energy resolution & & & \\
Timing resolution (tracker) [ps] & & & \\
Timing resolution (calorimeters) [ps] & & & \\
Timing resolution (muon system) [ps] & & & \\
Flavour tagging & & & \\
Boosted hadronic resonance ID & & & \\
\hline\hline
\end{tabular}
\end{center}
\end{table}

==> Chapters/P-PowerConverters/power.tex <==
\section{Power Converters}
\label{power:sec}
%% ==== START TentativeChapters/Author14-PowerConverters ==== %%
\subsection{Resistive magnets equivalent circuital model}
\label{power:sec:magnet_circuit}
At the present state, we are considering that all the resistive magnet length is occupied by dipole magnets. This approach is conservative for the power converters because dipole magnets have the largest energy density.  
Tab.~\ref{tab:PC_pars} reports the important parameters for the dimensioning of the power converters for the resistive magnets. 

\begin{table}[h]
\begin{center}
\caption{Important dimensioning values for the power converters of the RCS}
\label{tab:PC_pars}
\begin{tabular}{lcccc}
\hline\hline
  & {\textbf{RCS1}} & {\textbf{RCS2}} & {\textbf{RCS3}} & {\textbf{RCS4}} \\
\hline
Total length: lmag [km] & & & & \\
Max flux density: Bmax [T] & & & & \\
Airgap width: wg [mm] & & & & \\
Airgap height: hg [mm] & & & & \\
Magnets peak energy: Emag [MJ] & & & & \\
B ramping time: Tramp [ms] & & & & \\
Repetition times: Trep [ms] & & & & \\
Magnets inductance: Lmag [uH/m] & & & & \\
Magnets Resistance: Rmag [u$\Omega$/m] & & & & \\
Power converter peak power: Ppk [GW] & & & & \\
Power converter peak current: Ipeak [kA] & & & & \\
Power converter total output voltage: Voutpk [MV] & & & & \\
\hline\hline
\end{tabular}
\end{center}
\end{table}

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.6\textwidth]{TentativeChapters/Author14-PowerConverters/Figures/LinearRamp.png}
  \end{center}
\caption{Linear ramp}
\label{fig:PC_LinearBramp}
\end{figure}

Using Eq.~\ref{eq:PC_NRG} one can calculate the energy values reported in Tab. \ref{tab:PC_pars} for the case of an ideal linear ramp (see Fig. \ref{fig:PC_LinearBramp}). Similarly Eq.~\ref{eq:PC_Power} allows the calculation of the maximum power and output voltage that the power converters must supply.
\begin{equation}
\label{eq:PC_NRG}
E_{gap@B_{max}}=\frac{B_{max}^2}{2 \mu_0} l_{mags} h_{gap} w_{gap}, ~~~~~E_{mag}\approx 1.5 E_{gap@B_{max}}
\end{equation}
\begin{equation}
\label{eq:PC_Power}
P_{max}=\frac{2 E_{mag}}{\frac{T_{ramp}}{2}},~~~~~ V_{out}=L_{mag} \frac{di}{dt} +R_{mag} i
\end{equation}

\noindent The value of $R_{mag}$ reported in Tab.~\ref{tab:PC_pars} is the result of an electromagnetic Finite Element simulation of one of the analysed cases. $R_{mag}$ is strongly dependant upon the effects of eddy currents on both the coils and the iron of the resistive magnets and must therefore be calculated on an optimised design. 
The magnets equivalent circuit as the one reported in Fig. \ref{fig:PC_EquivCircuit} will then be used to design the power converters.
\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.8\textwidth]{TentativeChapters/Author14-PowerConverters/Figures/MagnetsEqCircuit.png}
  \end{center}
\caption{Magnet equivalent circuit }
\label{fig:PC_EquivCircuit}
\end{figure}

\subsection{Partition of the total power into different sectors}
\label{power:sec:sectors}
Given the extremely high power levels required for the acceleration, it is mandatory to distribute it in different independent sectors along the accelerator circumference. The concept is shown in Fig. \ref{fig:PC_Sectors} for the case where for every RF station we have two powering sectors. Each power sector is then divided into a given number (eigth in Fig. \ref{fig:PC_Sectors}) of parallel/series connected cells.
\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.8\textwidth]{TentativeChapters/Author14-PowerConverters/Figures/Sectors.png}
  \end{center}
\caption{Powering sectors and cells}
\label{fig:PC_Sectors}
\end{figure}
How each power cell is realized, is the object of the next paragraph.

\subsection{Power cell topologies}
\label{power:sec:topologies}
Despite distributing the total power across multiple cells connected in series or parallel (as shown in Fig. \ref{fig:PC_Sectors}), powering remains a complex challenge. Considering the anticipated high costs of the complete powering system, a promising strategy is to use natural resonance to achieve elevated peak powers. 
In this method, a natural resonance is triggered by connecting one or more pre-charged capacitor bank to the magnets, thus initiating an RLC resonance. This process can be repeated at a frequency of five Hz, aligning with the desired repetition rate. Two potential implementations of such a circuit are depicted in Fig. \ref{fig:PC_ResonatingCircuits} and are identified as "Full wave resonance" and "Switched resonance".
\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.8\textwidth]{TentativeChapters/Author14-PowerConverters/Figures/Power Cells Topologies.png}
  \end{center}
\caption{resonating circuits: full wave resonance (left), switched resonance (right)}
\label{fig:PC_ResonatingCircuits}
\end{figure}
The optimal design will emerge from comprehensive optimization computations. Each potential solution will be assessed based on the cumulative capacitive and inductive energy it requires to produce the intended resonant current within the magnets. 
For calculating the objective function, energy density values akin to those presented in Tab.~\ref{tab:PC_parsstorage} will be taken into account.

\begin{table}[h]
\begin{center}
\caption{preliminary dimensioning factor for the energy storage elements of the power converters for the RCSs}
\label{tab:PC_parsstorage}
\begin{tabular}{lcc}
\hline\hline
  & {\textbf{Full wave resonance}} & {\textbf{Switched resonance}} \\
\hline
Capacitor energy density: Cd [lt/kJ] & & \\
Capacitor energy floor occupation IP00: Co [$m^2$/kJ] & & \\
Capacitor energy floor occupation installed: Coi [$m^2$/kJ] & & \\
Inductor energy density: Ld [lt/kJ] & & \\
Inductor energy floor occupation IP00: Lo [$m^2$/kJ] & & \\
Inductor energy floor occupation installed: Loi [$m^2$/kJ] & & \\
\hline\hline
\end{tabular}
\end{center}
\end{table}

The values have been calculated starting from existing recent examples of high power converters where the energy storage concept has been used, namely the POPS (POwer for PS) power converter at CERN. It can be noted that according to the type of resonant circuit employed, the energy density in capacitors changes as a result of the voltage polarity reversal that forces the dielectric field to be smaller inside the capacitor dielectric film as illustrated by Eq. \ref{eq:PC_CapsNRG}.
\begin{equation}
\label{eq:PC_CapsNRG}
\begin{split}
Energy_{muCol}&=Energy_{pops} (\frac{\Vec{D}_{fullwave}}{\Vec{D}_{pops}})^2=274(\frac{80 \text{[V/$\mu$m]}}{250 \text{[V/$\mu$m]}})^2\approx 274 \frac{1}{10} \text{[J/lt]}\\
Energy_{muCol}&=Energy_{pops} (\frac{\Vec{D}_{switched}}{\Vec{D}_{pops}})^2=274(\frac{200 \text{[V/$\mu$m]}}{250 \text{[V/$\mu$m]}})^2\approx 274 \frac{1}{1.56} \text{[J/lt]}
\end{split}
\end{equation}
%rogers edit: \micro -> \mu. Looks like latex cannot parse siunitx within an equation


\subsubsection{The full wave resonance circuit}
\label{power:sec:fullwave}
The full wave resonance can be composed by either one, two or more parallel branches resonating with the magnets. One switch per branch ignite the resonance startig from pre-loaded capacitors and returning to the initial value (minus the losses of the system) at the end of the oscillation. 
\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.9\textwidth]{TentativeChapters/Author14-PowerConverters/Figures/FullWaveOscill.png}
  \end{center}
\caption{full wave resonance example}
\label{fig:PC_fullwaveexample}
\end{figure}
Fig.~\ref{fig:PC_fullwaveexample} show an example of a full wave resonance with two harmonics, the fundamental and the second. Because of the additional harmonics the total installed capacitive and inductive energy, is much higher that the energy required by the magnet at peak flux density. In addition the discharge of the capacitors is bipolar which poses significant overdimensioning constraints to the capacitors
The resonance parameters can be calculated using Eq. \ref{eq:PC_FullWave}
\begin{equation}
\label{eq:PC_FullWave}
\begin{split}
C_1&=\frac{1}{L_{mag}\omega_f^2 (1+n^2)-L_{mag} \omega_p^2}\\
C_2&=\frac{n^2\omega_f^4-n^2\omega_f^2\omega_p^2-\omega_f^2\omega_p^2+\omega_p^2}{n^2\omega_f^4L_{mag}(n^2\omega_f^2+\omega_f^2-\omega_p^2)}\\
L_2&=-\frac{L_{mag}(n^2\omega_f^2+\omega_f^2-\omega_p^2)^2}{n^2\omega)f^4-n^2\omega_f^2\omega_p^2-\omega_f^2\omega_p^2+\omega_p^4}\\
V_{C_10}&=L_{mag}\omega_f(I_{k1}+I_{kn}n)\\
V_{C_20}&=-\frac{L_{mag}n\omega_f^3(I_{k1}n^3\omega_f^2+I_{kn}n^2\omega_f^2-I_{kn}n\omega_f^2-I_{k1}n\omega_p^2+I_{kn}\omega_f^2-I_{kn}\omega_p^2)}{n^2\omega_f^4-n^2\omega_f^2\omega_p^2-\omega_f^2\omega_p^2+\omega_p^4}
\end{split}
\end{equation}

Where:
\begin{itemize}
\item $\omega_f$ \text{: is the main oscillation frequency;}
\item $\omega_p$ \text{: is one of the pole's frequency and is an additional dof;}
\item $n$ \text{: is the order of the additional harmonic;}
\item $I_{k1}$ \text{: is the required first harmonic peak value;}
\item $I_{kn}$ \text{: is the required nth harmonic peak value;}
\end{itemize}

\subsubsection{The switched resonance circuit}
\label{power:sec:switched}
In the switched resonance circuit, a distinct approach is employed. This method leverages two distinct simple resonances for different segments of the resonating wave, as depicted in Fig.~\ref{fig:PC_SwitchedParts}. To initialize the pulse, the preload capacitor (see Fig.~\ref{fig:PC_ResonatingCircuits}, right panel) is engaged until the current attains the target negative value. Subsequently, the current pathway is altered by toggling the switches S1 and S2, bringing the boost capacitors into operation.

\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.6\textwidth]{TentativeChapters/Author14-PowerConverters/Figures/SwitchedResonanceoscillationparts.png}
  \end{center}
\caption{Switched resonance principle}
\label{fig:PC_SwitchedParts}
\end{figure}

An example of transient with the switched resonance circuit is shown in Fig. \ref{fig:PC_Switchedexample} and the equations for dimensioning of the different components are reported in Eq.~\ref{eq:PC_Swiched}.
\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.9\textwidth]{TentativeChapters/Author14-PowerConverters/Figures/SwitchedResonanceoscillationexample.png}
  \end{center}
\caption{Switched resonance example}
\label{fig:PC_Switchedexample}
\end{figure}

\begin{equation}
\label{eq:PC_Swiched}
\begin{split}
I_{mag} &= I_0 e^{-\alpha t}\cos{\omega_d t}+\frac{Vc_0-I_0 \frac{R_{mag}}{2}}{L_{mag} \omega_d} e^{-\alpha t}\sin{\omega_d t}\\
V_c &= -L_{mag} e^{-\alpha t}\left[ \left( \frac{Vc_0-I_0 \frac{R_{mag}}{2}}{L_{mag} \omega_d}\alpha +I_0 \omega_d\right)\sin{\omega_d t}+\left(I_0\alpha -\frac{Vc_0-I_0 \frac{R_{mag}}{2}}{L_{mag} \omega_d}\right) \omega_d\cos{\omega_d t}\right]+R_{mag} I_{mag} \\
\end{split}
\end{equation}

Where:
\begin{itemize}
\item $I_0$ \text{: is the initial current in the magnet;}
\item $Vc_0$ \text{: is the initial voltage of the Cprelaod or Cboost capacitor banks;}
\item $\alpha = \frac{R_{mag}}{2 L_{mag}}$ \text{: is the time constant of the magnets;}
\item $\omega_d=\sqrt{\frac{1}{L_{mag} C_{preload/boost}}-\alpha^2}$ \text{: is the resonating frequency of either the preload or boost resonance;}
\end{itemize}


%% ==== END TentativeChapters/Author14-PowerConverters ==== %%

==> Chapters/S-Vacuum/vacuum.tex <==
\section{Vacuum}
\label{vacuum:sec}


==> Chapters/T-Cryogenics/cryogenics.tex <==
\section{Cryogenics}
\label{cryo:sec}

For the collider arc magnets (i.e. series production, multiple units), several design drivers have been identified.
Those are energy consumption, cryogenic availability, choice of conductor, local heat extraction, distribution losses, and reduced complexity.
Considering the various constraints imposed by these main drivers, which combine both sustainability and technical requirements, the main conclusions are stated in Table~\ref{cryo:tab:collider}.

\begin{table}
    \centering
    \begin{tabular}{c|cccc} 
         Parameter&  System&  Unit&  Value& Comments\\ \hline
         Overall power consumption &  Cryogenics of collider magnets&  kW/m&  & \\
         Temperature&  Absorber&  K&  & \\
         Heat load&  Coil&  W/m&  & \\
         Temperature&  Coil, cold mass&  K&  & \\
    \end{tabular}
    \caption{Fundamental design requirements for the cryogenic design of superconducting magnets for the collider ring.}
    \label{cryo:tab:collider}
\end{table}

==> Chapters/V-Costing/costing.tex <==
\section{Costing}
\label{cost:sec}

%% In discussion with Carlo Rossi
%% Information to be confirmed in September
%% Example (filler) below

The costing of the Muon Collider is directly dependent on a number of parameters contained within this report.
When performing cost optimization of various subsystems i.e. of the collider, it is important to consider the relative performance of the infrastructure, for example, magnets vs RF.
Below, Table \ref{cost:tab:collider} contains a list of parameters that have a direct impact on the cost optimization of the \SI{10}{\tera\electronvolt} collider.


\begin{table}[!h]
    \centering
    \begin{tabular}{cc|cc}
         Parameter&  Unit& Value & Impact on costing\\ \hline
         &  &  &\\
         &  &  &\\
         &  &  &\\
    \end{tabular}
    \caption{Cost-impacting parameters of the collider ring}
    \label{cost:tab:collider}
\end{table}

==> authorsnote.tex <==
\begin{tcolorbox}[colback=teal!10, colframe=teal!90, title=NOTES TO CONTRIBUTORS. PLEASE READ BEFORE EDITING]
Please refrain from adding numbers from the spreadsheet to the LaTeX document until we are on the Final Draft.
This is to prevent the LaTeX Version from straying from the Spreadsheet numbers whilst they continue to be updated and altered.
The editing link to the spreadsheet can be found here: \url{https://cernbox.cern.ch/s/VCI47bG4tSs9K8F}.\\

Want an easy way to copy tables from Excel to Overleaf?
Go to the Overleaf Visual Editor!
Tutorial available in Excel2LaTeX\_Tutorial.pdf attached in this Overleaf.\\

Looking for the text from last year's unpublished extended parameters report?
You can find it in the "TentativeChapters" folder.
Please do not edit these files directly. 
Only files in the "Chapters" folder will be added to the Parameter Report.\\

Adding extra packages?
Please define it in packages.tex, not in main.tex.\\

Sections are to be labelled  \textbackslash label\{secname:sec\}, where \textit{secname} = 'intro', 'front', 'highacc' etc.
Subsections are to be labelled as \textbackslash label\{secname:sec:subsecname\}.
Figures as \textbackslash label\{secname:fig:figname\}. 
Tables as \textbackslash label\{secname:tab:tabname\}.
Please follow the tab labelling scheme of the Spreadsheet.\\

Please use siunitx package as much as possible when defining units, for consistency. 
E.g. {\SI{10}{\tera\electronvolt}, \si{\tesla\per\meter\squared}, \num{2.99E8}} \\

(Style preference) Please write one sentence per LaTeX line, for readability. \\

Regarding bibliography: 
Please put references in bib/mybib.bib, or as a bibitem after \textbackslash begin\{thebibliography\}
 \end{tcolorbox}
 \clearpage



 %%%% Detector Table %%%%
 

\begin{table}
    \centering
    \begin{tabular}{ccccllllcccccc}
         Detectors&  \multicolumn{2}{c}{$R_{min}$}&   \multicolumn{2}{c}{$R_{max}$}& \multicolumn{2}{c}{$|Z|_{min}$}&\multicolumn{2}{c}{$|Z|_{max}$}&  Ang. Acc.&  \multicolumn{2}{c}{X / X0}&  \multicolumn{2}{c}{L / L0}\\
 Unit& \multicolumn{2}{c}{mm}& \multicolumn{2}{c}{mm}& \multicolumn{2}{c}{mm}& \multicolumn{2}{c}{mm}& deg& & & &\\
         Inner Trackers&  30&  28&   \multicolumn{2}{c}{1500}& \multicolumn{2}{c}{0}&\multicolumn{2}{c}{2300}&  10 -- 170&  \multicolumn{2}{c}{0.1 to 0.3}&  \multicolumn{2}{c}{0.04 to 0.1}\\
         \multicolumn{14}{l}{EM Calorimeter}\\
         - Barrel&  1857&  1690&   2124& 1960& \multicolumn{2}{c}{0}&2307&  2210&  10 -- 170&  42&  38&  1.9& 1.7\\
         - Endcap&  \multicolumn{2}{c}{310}&   2124& 1960& \multicolumn{2}{c}{2307}&\multicolumn{2}{c}{2577}&  &  40&  33&  1.8& 1.4\\
         \multicolumn{14}{l}{HAD Calorimeter}\\
         - Barrel&  2125&  2902&   4112& 4756& \multicolumn{2}{c}{0}&2575&  2609&  10 -- 170&  100&  89&  10.9& 9.5\\
         - Endcap&  \multicolumn{2}{c}{307}&   4112& 4756& \multicolumn{2}{c}{2575}&4562&  4434&  &  114&  116&  12.3& 12.5\\
         \multicolumn{14}{l}{Muon Systems}\\
         - Barrel&  4150&  4806&   7150& 6800& \multicolumn{2}{c}{0}&4565&  4444&  10 -- 170&  &  --&  & --\\
 - Endcap& \multicolumn{2}{c}{446}& 7150& 6800& 4565& 4444& 6025& 5903& & & --& &--\\
 Solenoid& 1500& 2055& 1857& 2862& & & 2307& 2509& --& 6& 18& 1.4&2.7\\
 Nozzle& \multicolumn{2}{c}{10}& \multicolumn{2}{c}{55}& & & \multicolumn{2}{c}{5950}& 0.2 -- 10& & --& &--\\
    \end{tabular}
    \caption{MAIA (left), MUSIC (right)}
    \label{tab:my_label}
\end{table}

